Learning from Informants: Relations between Learning Success Criteria

Learning from positive and negative information, so-called \emph{informants}, being one of the models for human and machine learning introduced by E.~M.~Gold, is investigated. Particularly, naturally arising questions about this learning setting, originating in results on learning from solely positive information, are answered. By a carefully arranged argument learners can be assumed to only change their hypothesis in case it is inconsistent with the data (such a learning behavior is called \emph{conservative}). The deduced main theorem states the relations between the most important delayable learning success criteria, being the ones not ruined by a delayed in time hypothesis output. Additionally, our investigations concerning the non-delayable requirement of consistent learning underpin the claim for \emph{delayability} being the right structural property to gain a deeper understanding concerning the nature of learning success criteria. Moreover, we obtain an anomalous \emph{hierarchy} when allowing for an increasing finite number of \emph{anomalies} of the hypothesized language by the learner compared with the language to be learned. In contrast to the vacillatory hierarchy for learning from solely positive information, we observe a \emph{duality} depending on whether infinitely many \emph{vacillations} between different (almost) correct hypotheses are still considered a successful learning behavior.

==> MapInfDelayableEx.tex <==
\newcommand{\drawBackboneTwo}{
\begin{scope}[every node/.style={minimum size=4mm}]

\node (nothing) at (0,0) {\textbf{T}};
\node (nu)  at (3,-1)     	{$\NU$};
\node (dec)  at (1,-3)   		{$\Dec$};

\node (smon) at (-5,-8)		  {$\SMon$};
\node (mon) at (-5,-6)		  {$\Mon$}; 
\node (wmon) at (-1.5,-3.5)     {$\WMon$};
\node (caut) at (-2,-2)    	{$\Caut$};

\node (sdec) at (3,-5)   		{$\SDec$};
\node (snu) at (5,-3)     	{$\SNU$};
\node (conv) at (5,-7)     	{$\Conv$};

\draw (smon) -- (dec);
\draw (snu) -- (nu);
\draw (nu) -- (dec);
\draw (dec) -- (sdec); 
\draw (sdec) -- (snu);
\draw (snu) -- (conv);
\draw (nothing) -- (caut);
\draw (caut) -- (smon);
\draw (nothing) -- (nu);
\draw (nothing) -- (wmon);
\draw (nothing) edge[bend right] (mon);
\draw (mon) -- (smon);
\draw[line width=8pt,draw=white] (wmon) edge[bend right=25] (conv);
\draw (wmon) edge[bend right=25] (conv);
\draw (wmon) -- (smon);
\end{scope}
}

\begin{figure}[h]
\begin{center}
\begin{minipage}{12cm}
\begin{tikzpicture}[above,sloped,shorten <=2mm,, shorten >=2mm]


\node[shape=rectangle,rounded corners,fill=lightgray] at (-5,-1) {$\Inf\Lim$};
\node[shape=rectangle,rounded corners,fill=lightgray] at (-5,-2) {$\Sd\Inf\Lim$};

\drawBackboneTwo

\node[line width=3pt, rounded corners, fit=(nu) (nothing) (dec) (snu) (sdec) (conv)] (Fit1) {};

\node[line width=3pt, rounded corners, fit=(nu) (nothing) (dec) (snu) (sdec) (conv) (wmon)] (Fit2) {};

\path[draw=lightgray,line width=3pt, rounded corners] (Fit1.north west) -- ([yshift=6.2mm] Fit1.west) -- ([yshift=6.2mm] Fit2.west) -- (Fit2.south west) -- (Fit1.south west) -- (Fit1.south east) -- (Fit1.north east) -- cycle;

\node[draw=lightgray,line width=3pt, rounded corners, minimum width= 15mm,minimum height = 8mm, anchor=center] at (mon) {};
\node[draw=lightgray,line width=3pt, rounded corners, minimum width= 15mm,minimum height = 8mm, anchor=center] at (smon) {};
\node[draw=lightgray,line width=3pt, rounded corners, minimum width= 15mm,minimum height = 8mm, anchor=center] at (caut) {};

\end{tikzpicture}
\end{minipage}
\end{center}
\caption{Relations between delayable learning restrictions in full-information (explanatory) $\Lim$-learning of languages from informant.}
\label{MapInfDelayableEx}
\end{figure}
